D-Bot: Database Diagnosis System using Large Language Models

Database administrators (DBAs) play an important role in managing, maintaining and optimizing database systems. However, it is hard and tedious for DBAs to manage a large number of databases and give timely response (waiting for hours is intolerable in many online cases). In addition, existing empirical methods only support limited diagnosis scenarios, which are also labor-intensive to update the diagnosis rules for database version updates. Recently large language models (LLMs) have shown great potential in various fields. Thus, we propose D-Bot, an LLM-based database diagnosis system that can automatically acquire knowledge from diagnosis documents, and generate reasonable and well-founded diagnosis report (i.e., identifying the root causes and solutions) within acceptable time (e.g., under 10 minutes compared to hours by a DBA). The techniques in D-Bot include (i) offline knowledge extraction from documents, (ii) automatic prompt generation (e.g., knowledge matching, tool retrieval), (iii) root cause analysis using tree search algorithm, and (iv) collaborative mechanism for complex anomalies with multiple root causes. We verify D-Bot on real benchmarks (including 539 anomalies of six typical applications), and the results show that D-Bot can effectively analyze the root causes of unseen anomalies and significantly outperforms traditional methods and vanilla models like GPT-4.

==> 02-preliminary.tex <==
%!TEX root = ../main.tex
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Large Language Models}

Large language models (LLMs) are a type of machine learning model specifically designed for natural language processing. Most of the current LLMs are based on Transformer~\cite{transformer} architecture, trained on gigantic unlabelled corpora through self-supervised learning tasks, thus possessing the power of understanding natural language. Since GPT-3~\cite{gpt3}, the LLMs are becoming remarkably stronger and have made significant strides in recent years. For instance, the recent ChatGPT~\cite{chatgpt} and GPT-4~\cite{gpt4} have exhibited possession of common sense knowledge, and outstanding ability to reason and perform logical inference tasks with high accuracy. This progress has led to an exponential increase in the number of applications of LLMs in various fields such as natural language generation, question-answering systems, and language translation, among others.

Meanwhile, as the language models become larger in size, their computational cost of large language increased dramatically. As a result, fine-tuning these large models for every downstream task has become impractical. This has sparked interest in a new approach to utilizing LLMs. Prompt-tuning is a general method that enables users to apply LLMs to new tasks and data domains without modifying the models themselves. This is achieved by incorporating prompts, such as descriptions, tags, and learnable components, as textual input to the LLM. Prompt-tuning is a powerful and efficient way of utilizing LLMs. In addition to prompt-tuning, the development of open-source LLMs like LLaMA~\cite{llama} has contributed to the flourishing of delta-tuning, an alternative method for utilizing LLMs. Delta-tuning involves adding extra parameters to the original LLM and updating only these additional parameters while keeping the LLM frozen. Since the number of tuned parameters is typically much smaller than the size of the original LLM, this approach reduces the computational cost and increases efficiency.

\subsection{\todo{???}}

==> 03-related_work.tex <==
%!TEX root = ../main.tex
\section{Related Work}
\label{sec:related_work}

\todo{Related Work}

==> 04-design.tex <==
%!TEX root = ../main.tex
\section{\sys System Design}
\label{sec:system-design}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.6\linewidth]{figs/abstraction.pdf}
  \caption{Abstraction illustration.}
  \Description{\sys consists of five layers of abstraction.}
  \label{fig:abstraction}
\end{figure}

The \sys system is designed with a five-layer abstraction to facilitate efficient and effective data science applications. The layers in a top-to-bottom hierarchy include user application, high-level logical operator, low-level logical operator, physical operator, and implementation.

Taking the task of extracting people's names from website titles as a specific example. The high-level logical operator is a data science functionality with certain generality. In this case, an \texttt{EXTRACT} operator, which is configured with specific parameters, such as task description, input/output specifications, and the object to extract (i.e., "names"), all of which could be set by the users in simple natural language.

However, applying one high-level logical operator to all scenarios through the same low-level implementation would not be efficient or effective. To address this, \sys provides multiple alternative choices of low-level logical operators, each offering a different logical implementation pipeline consisting of a series of physical operators. These physical operators are decoupled from their actual implementations, allowing \sys to automatically optimize each physical operator and compile each of them into different implementations depending on specific task instances. The compilation and debugging of the physical operators are completed mostly within the \sys system and boosted by the power of LLMs.

% \todo{Workflow illustration. Replace this one. System architecture + data flow (highlight components, inputs, outputs, separately).}

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/illustration.pdf}
  \caption{Illustration.}
  \Description{Users only need to communicate with \sys, while \sys coordinates LLMs, data, and tools to generate an efficient and effective local solution.}
  \label{fig:illustration}
\end{figure}

In the \sys study, various methods of employing LLMs in data science applications were investigated, focusing on two primary uses: direct query and code generation. Direct query treats each operator as a black-box function $f:X \to Y$, predicting the output $Y$ from input $X$ in zero-shot or few-shot settings. Code generation necessitates LLMs to create an executable program $r_f$ (e.g., in Python) that corresponds to $f$ for every input-output pair $(X,Y)$, expecting $r_f \equiv f$. The direct query typically assesses the effectiveness of incorporating LLMs, while code generation is employed for greater efficiency, as the executable $r_f$ runs locally. To further enhance LLM utilization, \sys employs a strategy that prioritizes localized computation through a series of optimizer modules: cacher, validator, simulator, ensembler, and adaptor. These modules allow \sys to develop an LLM-powered local solution for improved results. Additionally, \sys incorporates inter-operator optimizations such as predicate pushdown and path compression. Beyond primary uses, \sys explores other LLM applications, including suggestion, planning, and miscellaneous techniques to increase their utility. Furthermore, \sys tackles automatic local data processing with LLMs, encompassing data preprocessing for both LLMs and humans, data generation, and data annotation.

In subsequent chapters, we will examine each LLM utilization approach in detail and discuss specific techniques for optimizing LLM usage in relevant cases.

==> 04-prompt.tex <==
%!TEX root = ../main.tex



==> 05-feedback.tex <==
%!TEX root = ../main.tex



==> 05-optimization.tex <==
%!TEX root = ../main.tex
\section{Intra-operator Optimizations}
\label{sec:intra-optimization}

The optimization of each operator in \sys consists of a sequence of optimizer modules, namely cacher, validator, simulator, ensembler, and adaptor.

\todo{ordering: first introduction, then examples}

\subsection{Cacher}
\label{sec:cacher}

The cacher applies mainly for the direct querying of LLMs, as it is common to encounter numerous highly similar or even identical inquiries in the data. For a specific LLM, it provides similar or identical results for these inquiries, leading to inefficiencies in terms of repeated LLM calls. To address this issue~\cite{gpt-cache}, we introduced a cacher that leverages a small, frozen language model $\mathcal C$ to index and store the results of similar inquiries.

Consider the scenario of a web-content topic classification task. LLMs have demonstrated a remarkable capacity to accurately identify the subject matter of a given web content. As such, they could be employed as a potent instrument to directly address this challenge. However, to further improve their efficiency, LLMs can be utilized in an alternative manner - as annotators that identify and extract representative samples for each topic. By adopting this approach, the classification of new content can often be achieved by simply comparing it to the most similar examples, thereby reducing the need to rely on LLMs only for challenging cases. Furthermore, this approach ensured consistency in relation to the copious recurring content on the internet, which was showcased via replication, excerpts, and references. In \sys, the responsibility of storing these samples and recommending them based on their similarity lies with the cacher component.

Specifically, the cacher deploys $\mathcal C$ locally and creates an index for each input question $Q$ of the LLM using the vector output $\mathcal C(Q)$. The model is frozen so that the vector index is not changed. As the parameters of $\mathcal C$ are initialized by a pre-trained language model, $\mathcal C(Q)$ could provide a meaningful index without fine-tuning. In the aforementioned web-content topic classification example, we can simply cache $\mathcal C(\text{topic-classification} \oplus C)$ where $C$ denotes the web content and $\oplus$ denotes string concatenation with separators. For a more complicated example, to differentiate names from non-name noun phrases in the case of name extraction task, the cacher could use $\mathcal C(\text{name-extraction}\oplus T \oplus NP)$ to establish an index, where $T$ is the full-text passage and $NP$ is the proposed noun-phrase.

When a new inquiry is received, the cacher retrieves the top-$K$ most similar inquiries from the index to assist in processing the current inquiry. For classification problems, the cacher can directly obtain the result of the new inquiry through a majority ensemble, eliminating the need to query the LLM completely. For more open-ended questions, the top-$K$ similar inquiries can be integrated into prompts to the LLM, which can help improve the LLM's accuracy.

It is important to note that the cacher does not fine-tune the small language model $\mathcal C$. This is to ensure that the obtained vector $\mathcal C(Q)$ remains consistent for a fixed input $Q$ and can be stored. This guarantees the availability of conventional vector-based indexing techniques such as FAISS~\cite{faiss}, which allows the efficient retrieval of similar inquiries. If fine-tuning is required, a simulator (Sec.~\ref{sec:simulator}) may be more appropriate for optimizing this task. While it is possible to periodically fine-tune $\mathcal C$ to achieve more accurate semantic indexing, we do not recommend it as other optimizer modules such as a simulator can cover this functionality. The cacher primarily addresses efficiency and instant re-use.

Overall, the cacher is a practical approach to improving the efficiency and accuracy of LLMs in question-answering tasks. By leveraging the similarity between inquiries, we can reduce the number of repeated LLM calls and enhance the accuracy of the model.

\subsection{Validator}
\label{sec:validator}

Consider the scenario of tokenization, a seemingly simple task that can be implemented with just a few lines of code. However, complexities arise when dealing with letter cases, dates, punctuation, special characters, foreign languages, and so on. In specific situations, the behavior of a tokenization process must be clearly defined through examples and verified against these examples. In fact, for any operators, it is essential to guarantee their accurate and effective performance in executing their intended functions. This necessitates adherence to predefined specifications and requirements while minimizing errors and deviations from expected outcomes. To attain this degree of reliability and precision, \sys proposes introducing a validator that rigorously tests and debugs all operators, regardless of whether they are implemented by LLMs, generated by LLM codes, or manually written codes, among others.

The validator is versatile and can be used on any operator. Its primary function is to facilitate automatic testing and debugging of operators. Recent research~\cite{react,reflexion} on LLM interaction has highlighted the importance of providing error feedback to LLMs and explored the potential of utilizing LLMs to assist in delivering such feedback. However, the current state of research on LLM error correction remains in its early stages: the experience in error fixing, which has been refined through trial and error within a single data point, is difficult to generalize to new instances. Furthermore, a formal procedure for rectifying errors has yet to be established. In the \sys system, we have refined the error feedback and suggestion involving LLMs, developed a complete procedure for generic error fixing, and broadened their scope to include code generation and code debugging.

% \lei{In general it is NOT clear how validator works.}

The automatic validator we propose consists of the following main steps:

\todo{add illustration figure}

\begin{compactitem}
    \item {\textbf{Verifier}}: The verifier necessitates that operators supply examples during the operator definition process. It assesses the accuracy of the operator's execution and confirms if the results on the provided examples align with the expected outcomes. The verifier can be a standard verifier, which typically demands the operator's output results to match the provided examples exactly, or a custom verifier, which can be acquired by integrating a standard verifier with a custom operator that offers a more adaptable definition of output accuracy. Pre-existing operators in the \sys system are accompanied by their own examples, and in data preprocessing, the \sys system automatically extracts and generates examples (Sec.~\ref{sec:generation}).
    
    \item {\textbf{Advisor}}: The advisor module serves a function akin to the Reflection LLM in Reflexion~\cite{reflexion}. It proposes modifications for prompts (for direct queries) and code (for code generation/debugging) based on historical prompts, historical code/queries, examples, example results, and error types. The historical prompts and code are facilitated by the code generation operator, as mentioned earlier. Meanwhile, the verifier's execution result determines the examples, example results, and error types. The LLM receives the combined input and generates a plan to fix the code, either by reverting to a previous version or creating a new one. If the LLM suggests generating a new code version, it is asked to further provide high-level insights into the error's cause and potential generic fixes. These suggestions can be used for user-facing interactions or as reference points for subsequent validation steps. By default, the advisor module uses an LLM to produce suggestions, but manual suggestions can be employed as an alternative when validation repeatedly fails.
    
    \item {\textbf{Code Validator}}: The code validator in the automatic validator is only applicable to operators with code attached. It modifies the code based on various inputs, including historical prompts, historical code, examples, example results, and error types. Most of these inputs are also used by its predecessor, the advisor. Additionally, the code validator incorporates suggestions derived from the advisor. The LLM processes the combined information to directly generate a new code version based on the advisor's suggestions. After modification, the automatic validator starts a new validation round and re-evaluates the examples using the verifier and advisor, completing the overall validation mechanism.
    
    \item {\textbf{Prompt Validator}}: The prompt validator within the automatic validation system is primarily designed for LLM queries. It adjusts prompts by considering historical prompts, code, examples, example results, error types, and suggestions. Notably, it can function as a fallback mechanism for the code validator when validation repeatedly fails. In other words, if the advisor and code validator cannot generate code that is suitable for most or all examples after several validation rounds, the prompt validator can intervene to modify the initial prompt in the code generation configuration. This process generates a new version tree of codes, potentially reducing the need for human intervention in the advisor.
\end{compactitem}

In summary, the validator we propose is a powerful tool for testing and debugging operators. It is compatible with any operator. Its sub-components: verifier, advisor, code validator, and prompt validator, work together to provide comprehensive feedback and suggestions for improving the operator's performance.

\todo{add example tokenization}

\todo{elaborate}

\subsection{Simulator}
\label{sec:simulator}

The simulator is suitable for any operator with high execution costs. Unlike the cacher with static vector indexing, the simulator introduces a more complex encoding process that provides better flexibility and accuracy.

Consider the scenario of entity resolution. As previously mentioned in the introduction of the cacher (Section \ref{sec:cacher}), end-to-end LLMs may be capable of performing these tasks. However, they might not be as efficient as a localized solution. In the context of entity resolution, directly deploying a cacher to leverage historical queries may not be effective. This ineffectiveness can be attributed to several factors. First, the similarity measure used to determine whether two entities are identical is typically scenario-specific and unsuitable for a single frozen local model. Second, entity resolution places greater emphasis on the differences between query entities rather than their similarities, resulting in numerous potential false positives when using a naive similarity-based approach. Consequently, a tunable and adaptive measure is called for to localize the process of entity resolution effectively.

As mentioned above, any operator can be viewed as a black-box function $f: X \to Y$. The simulator continuously keeps track of the $(X,Y)$ obtained during online operation after the deployment of the data science application. When a pre-defined trigger is met (e.g., every $5000$ accumulated data records), the simulator re-trains a local model $\mathcal S_f$ to imitate the operator's behavior. The local model can then be used to replace the original operator when the accuracy or confidence exceeds a pre-defined threshold. It is important to note that the accuracy here does not represent the accuracy of the actual function to the ground truth, but rather the degree of agreement with the original operator's execution results. Using the local model $\mathcal S_f$ instead of the original operator can improve efficiency if the execution cost of the original operator is higher than that of the local model.

% \lei{Given a task, who and how to decide which model to use? No parameter tuning is needed?}

\todo{tuned large model add another section: details about LoRA}

The \sys system applies different types of local models depending on the input and output $(X,Y)$. Available choices are as follows:
\begin{compactitem}
    \item {\textbf{Small Language Model}}: A locally deployed sequence-to-sequence (Seq2Seq) model is the most common type of local model for simulating any serializable input $X$ and output $Y$. It is trained on self-supervised learning tasks such as autoregression on all collected data $(X \oplus Y)$ and can be used for conditional generation at inference time given $X$. Note that the encoder of the small language model can also be used for other purposes such as generating a vector representation of $X$ (more flexible and fine-tunable than the cacher, but not suitable for indexing regarding efficiency). Therefore, this tunable small language model can be used with shared parameters across multiple related modules.
    
    \item {\textbf{Tuned Large Model}}: The emergence of open-source LLMs such as LLaMA~\cite{llama} has made it possible to locally fine-tune LLMs. However, fine-tuning LLMs is an expensive process. Recent research has developed delta-tuning techniques such as LoRA~\cite{lora} to tune local LLMs. The LoRA technique introduces a low-rank matrix added to the original model parameters, which is updated instead of the original parameters during the tuning process. As the matrix is assumed to be low-rank, it can be represented by a decomposition matrix and a dimension-expansion matrix, both of which are much smaller than the original parameter matrix. This method can significantly reduce the number of parameters that need to be updated in tuning large language models and is therefore widely used. It is worth noting that the LoRA technique can not only be used for tuning LLMs but has also been applied in vision models~\cite{sd}. The simulator based on fine-tuned large models provides potential support for optimizing multi-modal data science applications within the \sys system.
    
    \item {\textbf{Classification Model}}: For cases where $Y$ has only a small number of categories, a classification head with an arbitrary encoder structure can be used as a local model for supervised learning. A classification model usually achieves better results than a universal sequence-to-sequence model. Furthermore, when instructed by the user, \sys simulator could cluster similar operator outputs to enable the usage of a classification model.
    
    \item {\textbf{Regression Model}}: For cases where $Y$ mainly contains numerical outputs, a regression head with an arbitrary encoder structure can be used as a local model for supervised learning. However, learning for regression problems with unstable numerical ranges can be difficult and is not recommended.
    
    \item {\textbf{Conventional Model}}: In data science, it is common for both $X$ and $Y$ to mainly consist of numerical or categorical features. More traditional machine learning methods such as linear regression, polynomial regression, elastic net regression, support vector machines, decision trees, XGBoost, etc. These methods have stronger interpretability but lower flexibility. Therefore, conventional models are not automatically applied by the \sys system and mainly rely on users with programming experience to choose.
\end{compactitem}

In practice, simulators operate almost autonomously: \sys utilizes a classification model for outputs with limited categorical values and a regression model for numerical outputs. For other scenarios, the small language model acts as a default option, unless the user specifically selects a tuned large model or a traditional model. By default, simulators apply only to direct query operators, unless stated otherwise, since generated or manual code is more efficient than machine learning models in most cases.

Apart from the local model choice and implementation, another important issue worth paying attention to is the control logic to determine when to substitute the original operator with the local model and when to stick to the original operator. The most straightforward strategy is to set a global threshold (e.g., $90\%$): whenever the accuracy of the local model is higher than the threshold, the local model completely bypasses the execution of the original operator.

However, various data points within the same task often exhibit differing levels of complexity. For instance, in named entity extraction, as previously mentioned, "Lincoln" is an ambiguous term that could represent multiple entities, whereas "Emily" is almost certainly a human name. Another example can be found in entity resolution; while most entities can be deduced through traditional similarity measures, identifying that "IBM" and "Big Blue" represent the same company is challenging without employing the common sense embedded in LLMs\footnote{"Big Blue" is the nickname of IBM, named after its blue logo.}. Consequently, a more efficient replacement method should rely on the confidence of the local model concerning the relevant data points.

\todo{as an independent section}

Most local models could obtain confidence indicators as a byproduct of their execution. For example, for classification models, the probability of the class with the highest predicted probability can be regarded as a confidence indicator: the closer the probability of the class with the highest predicted probability is to $1$, the higher the prediction confidence. For language models, the perplexity of the generated text can also be regarded as a confidence indicator: the lower the perplexity, the higher the prediction confidence. However, it should be emphasized that the confidence indicators provided by the model itself are empirical and cannot provide theoretical guarantees for the accuracy of the model. A non-robust model may output incorrect predictions with high confidence. Another commonly used confidence criterion is achieved through ensembles, for example: training multiple models with different initializations, and the number of models obtaining the majority classification on a data point can be regarded as a confidence indicator.

\todo{Technique: induce confidence from LLM API}

It is important to highlight that simulators can not only enhance the execution efficiency of operators but also increase their accuracy. In a teacher-student paradigm, it is commonly believed that the performance of a student model (in this case, the local model) is limited by its teacher model (in this case, the original operator). However, research~\cite{bootstrapping,bootstrapping2,distillation,toolformer} has demonstrated that a student model, obtained through self-training on the filtered output of the teacher model, may outperform the teacher model, a phenomenon known as bootstrapping. This occurs because filtering the teacher model's output and retaining only high-confidence data results in slightly higher-quality training data for the student model compared to the raw data used by the teacher model. Furthermore, since the local model can continuously learn the real data distribution after deployment by the data custodian and adapt to manually corrected erroneous labels, it can progressively surpass the original static operator over time.

\subsection{Ensembler}
\label{sec:ensembler}

In the majority of data science applications with verifiable outputs, such as classification problems (e.g., entity resolution and topic classification) with clearly defined ground truths, employing an ensemble of multiple models can potentially lead to superior outcomes compared to relying on a single model.

The role of the ensembler involves generating various diverse models and pinpointing the most effective ones with the assistance of validator modules. Owing to the substantial disparity in computational complexity between direct query and code generation, these methods are typically ensembled independently.

Regarding the integration of LLMs into the ensemble, in the context of the direct query, the ensembler promotes diversity in the initial prompt and the prompt validator. More specifically, the LLM is responsible for rephrasing the prompts to produce alternative results. In the context of code generation, the ensembler focuses on the initial prompt and code validator, requiring the LLM to implement the provided function in distinct ways. In addition to employing LLMs, operators with verifiers also facilitate diversification based on the chosen failure cases.

\todo{pseudo-code on genetic algorithm}

The ensemble method incorporates the majority voting ensemble as its simplest yet most adaptable technique. Additionally, using an accuracy-weighted voting strategy provides a more versatile solution with the ability to exclude low-accuracy candidates. Specifically, a predetermined number $M$ of prompt and code variations are generated through LLM-advised prompts or randomly selected failure cases from the verifiers during each iteration. The top $m < M$ variations are preserved and employed to generate the next iteration of variations. This method is akin to the genetic algorithm, wherein variants are created, assessed, chosen, and mutated. In addition to evaluation and selection based on a fixed set of examples provided by the operator, it is feasible to use data generated by LLMs (Sec.~\ref{sec:generation}) or data annotated (Sec.~\ref{sec:annotation}) post-deployment to further enhance the ensemble process. Beyond accuracy as a criterion, it is also possible to employ a confidence indicator as a dynamic voting weight, as suggested in the simulator section (Sec.~\ref{sec:simulator}).

In most cases, a standard ensembler employed for classification tasks does not introduce additional complexity beyond a minor constant, as the aggregation strategy is straightforward and the ensembled variations exhibit comparable computational complexity levels. However, when striving for improved performance and efficiency is not a limiting factor, employing an LLM ensemble method becomes a viable option. This technique treats the individual outputs as alternatives or components presented in the prompt and the LLM is asked to select a single option or construct more complex responses based on the provided components. Moreover, the ensembler is allowed to create ensembles containing methods of different computational complexity if and when explicitly required.

\todo{rename}
\subsection{Adaptor}
\label{sec:adaptor}

The adaptor in \sys typically serves as an interface that enables the LLMs to access local data and existing data science tools, thereby bridging the gap between these resources and the LLMs' capabilities.

Consider the scenario of NL2SQL, which involves converting natural language queries into SQL queries for a specific database. On the one hand, it is generally both insecure and inefficient to provide the entire database as input to the LLM. On the other hand, supplying only the table schema could restrict the LLM's ability to generate SQL queries with correct predicate values. To address similar challenges in presenting local data and local tools to LLMs, a unified and enhanced approach is necessary.

The adaptors comprise the following main types:
\begin{compactitem}
\item {\textbf{Custom Operators}}: Utilizing a modularized approach, both built-in and user-defined operators in \sys can act as building blocks for new user-defined operators. Specifically, for any operator $f:X \to Y$ defined within the \sys system, the adaptor generates a description $(d_f, d_X, d_Y)$ about the operator, input, and output to be provided to LLMs, as well as an API for $r_f$ in a specified programming language, such as Python. As a result, the adaptor can be invoked by the LLMs through interaction or by code generated by the LLMs.

\item {\textbf{Custom Data Science Tools}}: Given the diverse nature of data science applications, it is often more efficient and effective to incorporate existing data science tools as a single step within a comprehensive data science application. For instance, when analyzing periodic time series data, providing FFT as an available tool can streamline code generation by LLMs and enhance their ability to develop a more effective data science application. For widely used public data science tools, LLMs can already leverage their power as they are present in the code contained in the pre-training corpora. However, for private packages, users can provide the description $(d_f, d_X, d_Y)$ about the tools, as \sys does for built-in operators. Alternatively, users can supply use cases or documentation, which can then be fed to the LLMs to automatically generate the description $(d_f, d_X, d_Y)$. While the latter approach is more convenient, its effectiveness is not guaranteed.

\item {\textbf{Local Data}}: One of the most vital roles of the adaptor is to enable access to local data. Local data in data science applications can be extensive, private, and organized in various ways. As a result, the interface for accessing local data should be interactive, privacy-preserving, and unified. \sys provides built-in adaptors of this type, including Long Text Adaptors, Knowledge Graph Adaptors, Search Engine Adaptors, SQL Adaptors, etc., which serve as intermediate components between the LLMs and users. Users can set up any local server to respond to queries posted by the adaptors, and the adaptors should manage the process of handling queries and sending responses to the LLMs. Privacy is preserved under the control of the local server, while interaction and unification are achieved by the adaptors' implementation. More details about how adaptors efficiently intervene in the process of data access are discussed in Section \ref{sec:pre-processing}.

\item {\textbf{Workspace}}: The concept of utilizing memory to enhance the capabilities of LLMs has been a topic of interest in recent works~\cite{autogpt,langchain,recurrentgpt,scm}. These studies primarily treat memory as preserved textual prompts within a single dialogue, which can limit the scope of information retention and retrieval. In contrast, \sys introduces a more advanced and flexible workspace adaptor, which allows for memory storage in the local environment, thereby expanding the LLMs' capacity to manage and access information. Specifically, the workspace adaptor enables LLMs to store information as key-value pairs, which can be retrieved later as needed. \sys provides key-based value retrieval, similar key retrieval, and key listing to retrieve the stored information. Key-based value retrieval allows LLMs to access specific information directly by referencing the associated key, while similar key retrieval enables the identification and retrieval of related information based on key similarity. Additionally, key listing provides an overview of all existing keys in the local storage, facilitating easier navigation and management of stored information. By implementing the workspace adaptor, \sys allows LLMs to update and maintain information persistently even after the online deployment of the data science application. This enhanced memory management capability not only improves the efficiency and effectiveness of LLMs but also enables them to handle more complex tasks and develop more robust data science applications.
\end{compactitem}

The adaptors, which enable the integration of pre-defined operators, data science tools, and access to local data and storage, serve as crucial components in the \sys system for enhancing the efficiency of these operators.

\section{Inter-operator Optimizations}
\label{sec:inter-optimization}

Inter-operator optimization offers a substantial potential for enhancement in data science applications, going beyond the optimization of individual operators. The main goal of this optimization is to improve the overall planning and coordination of operators while preserving the modularity of treating each operator as a separate black box. This approach mainly concentrates on the organization and integration of operators. By broadening the optimization scope beyond a single operator, a more holistic and efficient strategy can be implemented for a wide array of prevalent data science applications.

To optimize a diverse data science application, it is crucial to focus on the bottleneck components, as each component may display different levels of computational complexity. The \sys system classifies operators based on their computational complexities, which consist of:

\begin{compactitem}
    \item {\textbf{Massive}}: This complexity level involves an operator that is considerably more costly than an LLM API call, typically necessitating the processing of a vast amount of local data to answer a single query.
    \item {\textbf{Significant}}: This level of complexity is analogous to an LLM API call.
    \item {\textbf{Moderate}}: Often representing the execution of a local machine learning-based solution or a data science tool. This complexity level is faster than an LLM API call but slower than straightforward data processing.
    \item {\textbf{Low}}: Basic processing of data. This complexity level is more or less comparable to scanning the data record.
    \item {\textbf{Minimal}}: Generally sub-linear. This level of complexity enables answering a query without processing the entire data required by the query.
\end{compactitem}

The inter-operator optimizations in \sys primarily involve substituting high-category operators with lower-category operators and absorbing lower-category operators into higher-category ones.

By focusing on the optimization of bottleneck components in a data science application, the system can effectively handle the diverse computational complexities of each component, leading to improved overall performance.

\todo{add section: cite volcano, pipeline execution scheme}

\subsection{Predicate Pushdown}
\label{sec:predicate-pushdown}

In numerous data science applications, it is often anticipated that data analysis will be conducted on a specific subset of the available data. As a result, identifying and isolating this filtered data at the earliest opportunity could lead to the elimination of the need for running computationally heavy operators thereby significantly improving computational efficiency.

In \sys, a special type of operator, the filter operator is designated for reducing the number of data records based on a condition, which could be either a simple expression or more general, the execution result of a custom operator. Consider describing the dependency of operators as a tree structure, the objective of predicate pushdown is to move the filter operator downwards as close to the raw data source as possible, most importantly before the execution of operators with high computation complexity.

The most direct and comprehensive approach involves employing a learning-based method to predict the filter predicate. This concept has previously been introduced in the simulator section (Sec.~\ref{sec:simulator}), where a local model is trained on deployed data to replicate the execution outcome. In this context, a local model is developed for each filter operator that has at least one massive, significant, or moderate operator preceding it in the pipeline. The purpose of this model is to predict whether the data should be discarded before reaching the computationally expensive operators.

In more complex cases involving predicate decomposition, the \sys system conducts a greedy search for each subtree with the filter operator as the root, aiming to identify the maximum block that can be bypassed accurately. Initially, only the filter operator is included in the subtree to be bypassed. After deployment, \sys collects data online and maintains a record of the average running time for each operator. Utilizing these statistics, the \sys system attempts to dynamically expand the tree. During periodic local model training, the system evaluates whether adding another layer of children or incorporating a specific child with a high average running time to the current subtree could produce a local model that meets the threshold for filtering out data.

\todo{add illustration figure}

This approach addresses the potential pushdown of placing filter predicates beneath moderate-complexity operators. The remaining need for further pushdown of predicates involves replacing low-complexity filters with minimal-complexity filters. Given the diverse nature of data science applications, such filters should be managed in conjunction with the \texttt{LOAD\_DATA} operator (Sec.~\ref{sec:pre-processing}), guided by human input and converted by the \sys system.

\subsection{Operator Compression}
\label{sec:operator-compression}

As opposed to the predicate pushdown in \sys, which typically replaces groups of high-complexity operators with a single moderate complexity operator (a learning-based local model), the operator compression in \sys mainly absorbs low-complexity operators with the high-complexity operators above and beneath it in the execution pipeline.

Specifically, for any operator that does not require a large amount of local data (non-massive operators), using an LLM query as a black-box simulator is viable. In general, an LLM query is highly resource-intensive, rendering such a simulation unworthy. However, when a significant-complexity operator is already present in the pipeline, it becomes feasible to employ an LLM to mimic an operator with similar computational complexity while simultaneously extending it to its related predecessors and successors, thereby marginally enhancing the overall running time.

\section{Data Processing}
\label{sec:processing}

\todo{split data processing into other sections?}

In the rapidly expanding field of data science, researchers often find themselves dedicating a substantial portion of their time and effort to preprocessing the heterogeneous data they encounter. The preprocessing stage, therefore, serves as a crucial step in transforming raw data into a clean, well-structured format for further analysis. With the help of LLMs, \sys has developed multiple methods in improving the processing and understanding of user-specified local data.

\subsection{Automatic Preprocessing}
\label{sec:pre-processing}

Firstly, when assuming that a portion or all of the local data is homogeneous and in a serializable format, the system can directly utilize the code generation operator to specify a \texttt{LOAD\_DATA} operator. For more complex cases, the \texttt{LOAD\_DATA} operator can be enhanced by validators (Sec.~\ref{sec:validator}), particularly the advisors, which serve as another LLM capable of explaining the data format and consequently provide a natural language guide for the code generation of the \texttt{LOAD\_DATA} operator.

However, in numerous instances, the potential input data size surpasses the context length of most existing LLMs. Moreover, considering efficiency and security concerns, local data should be presented to the LLM using a specified protocol. In the \sys system, a data processing protocol necessitates users to establish a local server with designated APIs that can be accessed by the LLM via adaptors, acting as the client. Defining such APIs may be an unnecessary task for simple data science applications; therefore, the system has established several protocols for common data science scenarios.

\subsubsection{Processing of Long Textual Data}
\label{sec:long-text}

\subsubsection{Processing of Knowledge Graphs}
\label{sec:knowledge-graphs}

\subsubsection{Data as Local Search Engine}
\label{sec:search-engine}

\subsubsection{Data as Structured Database}
\label{sec:sql}

\todo{}

\subsection{Generation}
\label{sec:generation}

\todo{}

\subsection{Annotation}
\label{sec:annotation}

\todo{}



==> 06-methodology.tex <==
%!TEX root = ../main.tex
\section{Operators}
\label{sec:methodology}

\todo{Fix context: after optimization}

As shown in Fig.~\ref{fig:architecture}, the core function of each physical operator relies on an LLM core. \sys compile a configuration $c$ needs to an executable $e$. In the case of directly querying LLM, the configuration is compiled into an initial prompt for every input instance and the resulting executable is an interactive dialogue between the \sys system and the LLM. In the case of code generation, the configuration is compiled into a program (e.g., in Python) once and could be applied efficiently for loads of inputs.

\subsection{Direct Query}
\label{sec:direct-query}

Any procedure inside a data science application could always be viewed as a black-box function $f: X \to Y$. A straightforward approach to utilizing LLMs is to directly request $Y$ given $X$. This end-to-end method is effective for most cases, particularly when the task is simple but requires domain-specific knowledge.

For direct LLM queries, the configuration $c_{DQ} = (P,d_t,d_i,d_o,E,A,V)$ comprises a prompt template $P$, a natural language task description $d_t$, input and output type descriptions $d_i$ and $d_o$, an optional list of examples $E$, an optional set of adaptors $A$ (Sec.~\ref{sec:adaptor}), and an optional list of validators $V$. Given a new input $i$, the configuration parses $P$ using $d_t,d_i,d_o,E,A$, and $i$ to generate an initial prompt $p_i^0$ for the LLM. The final LLM response is validated by $V$ and then used as the output after one or multiple rounds of interaction.

The default standard prompt template $P$ involves a single interaction round, where the LLM directly provides the desired output. However, for more complex tasks, the LLM may require additional planning and reasoning. Chain-of-Thought Prompting (CoT)~\cite{cot} addresses this by explicitly guiding LLMs through intermediate thinking steps before reaching a conclusion. During this process, the LLM sequentially appends $p_i^1, p_i^2, \cdots$ to the initial prompt $p_i^0$ until a successful final confirmation $p_i^j$ is made.

Multi-round interactions can also enable the use of external tools. Naïve CoT prompting generates a static plan, which cannot leverage environmental knowledge. ReAct~\cite{react} addresses this by formulating multi-step reasoning with interaction as thoughts, actions, and observations. Actions execute plans, observations represent environmental feedback, and thoughts are internal actions that do not affect the environment. Reflexion~\cite{reflexion} extends ReAct by incorporating a reinforcement learning-based procedure, introducing a second LLM as an instructor that provides heuristics based on the actor LLM's actions and environmental rewards. The actor LLM can then use these heuristics to improve its planning and actions.

In \sys, the system interacts with the LLMs by providing adaptors (Sec.~\ref{sec:adaptor}) that serve as interfaces for LLMs to access local data and conventional data science tools, and validators (Sec.~\ref{sec:validator}) that provide feedback on the correctness of LLM responses. This design enables the further extension of the Reflexion pipeline, with adaptors supplying observations and validators offering environmental rewards and heuristics.

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/direct_query.pdf}
  \caption{Direct Query: An NL2SQL Example.}
  \Description{...}
  \label{fig:direct-query}
\end{figure}

\sys supports three types of prompt templates: standard prompt, CoT prompt, and fully-interactive prompt. The standard prompt is sufficient for simple tasks and is used as the default when no adaptors are provided. For complex tasks, a CoT prompt can be employed to enhance effectiveness. However, in most cases, when adaptors are available, \sys utilizes the fully-interactive prompt to coordinate between the LLM and local data. Specifically, the initial prompt $p_i^0$ is generated with additional information provided: the set of available adaptors $A$. During each interaction round $j$, given $p_i^0,p_i^1,\cdots,p_i^{j-1}$, the LLM first generates thought $t_i^j$ and action $a_i^j$. The action either involves invoking an adaptor from $A$ or confirming the final response. An observation $o_i^j$ is returned, which could be the local data or function supplied by the invoked adaptor. Consequently, $(t_i^j,a_i^j,o_i^j)$ together form the next prompt $p_i^j$. Finally, the list of validators $V$ would provide feedback $S$ in case of an incorrect final response to refine the initial prompt $p_i^0$. (Fig.~\ref{fig:direct-query})

\subsection{Code Generation}
\label{sec:code-generation}

In addition to directly querying LLMs for accessing their common sense knowledge, another way to leverage LLMs is through code generation. This approach enables the swift and adaptive development of new data science applications. While direct querying of LLMs can be effective, it may not be feasible to process every data record using LLMs in certain sub-processes of a data science application that involve a massive amount of local data. Compared to directly querying LLMs, employing LLM-generated code locally can be more efficient. Compared to manually written code, LLM-generated code offers enhanced flexibility, as it can adapt to changing requirements and data formats.

However, most mainstream LLMs are not yet suitable for producing complex logic or building large-scale applications, as they are only capable of generating small pieces of code. To address this scalability issue, \sys emphasizes modularization and tool utilization to connect separate code pieces.

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/code_generation.pdf}
  \caption{Code Generation: A Name Extraction Example.}
  \Description{...}
  \label{fig:code-generation}
\end{figure}

For code generation, the configuration $c_{CG} = (P,d_t,d_i,d_o,E,A,V)$ is compiled into a local program function $r(\cdot)$, which can be independently applied to a list of inputs to obtain the corresponding outputs $o = r(i)$. Similar to directly querying LLMs, the configuration parses $P$ into the initial prompt $p_i^0$. The key difference is that the code of program $r$ is returned by the LLM with all the adaptors already considered. The subsequent interactions come from the validators $V$, whose feedback as well as the current program $r$ together compose the prompts $p_i^j$ to revise the generated code. (Fig.~\ref{fig:code-generation})

The significance of tool utilization in LLM-generated code cannot be overstated. As a crucial area of research, tool utilization has been gaining attention alongside recent advancements in LLMs. Previous studies~\cite{visual-chatgpt,hugginggpt} have primarily concentrated on prompt engineering to tackle the planning and decision-making aspects of tool utilization. However, in our context, high-level logical operators and user instructions predominantly dictate the planning process. Consequently, a more pressing concern is to accurately define and describe the tools.

In our \sys, tools encompass: open-ended tools, which refer to publicly available resources that LLMs can access, such as common Python packages; user-provided tools, which include APIs for local data science functions; and custom operators. LLMs inherently support open-ended tools through their pretraining process, while in \sys, user-provided tools and custom operators are managed via adaptors.

It is important to note that the code generation process in \sys not only produces a single piece of code in textual format but also records additional information to facilitate advanced modifications to the code. In technical terms, a generated executable comprises a list or tree of versions, where each version includes the code, linked to a specific programming language (such as Python), and the corresponding prompt used for generating that version. The preservation of historical code and prompts not only allows for efficient version control but also enables the integration of validators (Sec.~\ref{sec:validator}) and ensemblers (Sec.~\ref{sec:ensembler}) to improve the overall performance.

==> 07-future.tex <==
%!TEX root = ../main.tex


%todo
\section{Other Opportunities}
\label{sec:opportunities}


==> 07-processing.tex <==
%!TEX root = ../main.tex
\section{Data Processing}
\label{sec:processing}

In the rapidly expanding field of data science, researchers often find themselves dedicating a substantial portion of their time and effort to preprocessing the heterogeneous data they encounter. The preprocessing stage, therefore, serves as a crucial step in transforming raw data into a clean, well-structured format for further analysis. With the help of LLMs, \sys has developed multiple methods in improving the processing and understanding of user-specified local data.

\subsection{Automatic Preprocessing}
\label{sec:pre-processing}

First of all, when assuming that the local data, or a part of the local data is homogeneous and in serializable format, \sys could directly use the code generation operator to specify a \texttt{LOAD\_DATA} operator.

\subsubsection{Processing of Long Textual Data}
\label{sec:long-text}

\subsubsection{Processing of Knowledge Graphs}
\label{sec:knowledge-graphs}

\subsubsection{Data as Local Search Engine}
\label{sec:search-engine}

\subsubsection{Data as Structured Database}
\label{sec:sql}

\todo{}

\subsection{Generation}
\label{sec:generation}

\todo{}

\subsection{Annotation}
\label{sec:annotation}

\todo{}


==> 08-implementation.tex <==
%!TEX root = ../main.tex
\section{Implementation Details}
\label{sec:implementation}

\todo{Implementation Details: Python sandbox, prompt details, etc.}

==> 09-experiments.tex <==
%!TEX root = ../main.tex
\section{Experiments}
\label{sec:exp}

\todo{quantitative experiments: accuracy, efficiency, \#llm calls}

\todo{ablation on the core components}

\todo{multiple tasks: topic classification, imputation, entity resolution, NL2SQL, fancy example (map?), extraction (evaporate?), database operation}

==> 10-conclusion.tex <==
%!TEX root = ../main.tex
\section{Conclusion}
\label{sec:conclusion}

\todo{Conclusion}

\todo{Limitation}
